Glass-Vault: A Generic Transparent Privacy-preserving Exposure Notification Analytics Platform

The highly transmissible COVID-19 disease is a serious threat to people's health and life. To automate tracing those who have been in close physical contact with newly infected people and/or to analyse tracing-related data, researchers have proposed various ad-hoc programs that require being executed on users' smartphones. Nevertheless, the existing solutions have two primary limitations: (1) lack of generality: for each type of analytic task, a certain kind of data needs to be sent to an analyst; (2) lack of transparency: parties who provide data to an analyst are not necessarily infected individuals; therefore, infected individuals' data can be shared with others (e.g., the analyst) without their fine-grained and direct consent. In this work, we present Glass-Vault, a protocol that addresses both limitations simultaneously. It allows an analyst to run authorised programs over the collected data of infectious users, without learning the input data. Glass-Vault relies on a new variant of generic Functional Encryption that we propose in this work. This new variant, called DD-Steel, offers these two additional properties: dynamic and decentralised. We illustrate the security of both Glass-Vault and DD-Steel in the Universal Composability setting. Glass-Vault is the first UC-secure protocol that allows analysing the data of Exposure Notification users in a privacy-preserving manner. As a sample application, we indicate how it can be used to generate "infection heatmaps".

==> CrowdNotifier.tex <==
\section{Example: CrowdNotifier}
% citation: waiting for PoPETS21 issue 4 to be merged in cryptobib
\cite{} proposes crowdNotifier, a presence tracing system to detect contacts within an indoors venue. The implementation relies on a identity based encryption scheme, where each venue is a key generation authority. When a user checks in (using a QR code), the venue encrypts a ciphertext under the (user, time) identity. If an infection is recorded at a certain time, the venue releases the secret key for all users at that time.

We can reimplement CrowdNotifier using our system, by slightly stretching our previous assumptions. We let each venue act as a trusted keygen authority within the FESR scheme (or as proxies to a unique central trusted authority). Users checking into a venue register as auditor, by obtaining a functional key for the function ``Was there an infected case at venue x,time t?'' for the current time and venue (the keygen authority needs to be able to issue keys only for x). Infected users will then upload a list of venues they registered at, and their time of entry (and probably exit). Only users that where at the same venue at that time will obtain a return value from decrypting this ciphertext. Malicious users can upload arbitrary venue/time pairs, so FakeReality needs to move them to those locations but with antenna tp set to 0 (to show that regular exposure notification would not capture them).

(extensions: maybe venues sign some proof of location so no malicious data can be uploaded)


scalability: linear to constant?


==> auditing.tex <==
\section{Adding Auditing to contact tracing}
\subsection{Overview}
Our goal is to extended a decentralised contact tracing protocol with an
auditing interface, such that a third party is able to compute a function on
some shared global data over the protocol participants who have chosen to share
their infection status. To enable a wider class of functionalities to be
evaluated, beyond the simple proximity guaranteed by recording other users
chirps, we extend the ShareExposure input to take an additional set of
``secret'' inputs. These can correspond to a user's PII (age, health status),
geolocation, environmental reading (air humidity etc.), programs running on
their smartphone, level of noise in the room etc. As this data can encode
potentially sensitive information, it is important that it remains confidential
to the user who uploaded it. Thus, part of our security guarantees
shall be that a third party auditor can not learn an individual user's secret
input from the result of the functional evaluation. From a modelling
perspective, we simply mark some records in the user physical reality data
structure as $\phyrecsec$; these would not be returned to the user as part of
the $\textsc{MyCurrentMeas}$ call, to preserve post-compromise security.

Both the contact tracing protocol and exposure notification ideal
functionalities are now extended with two additional procedures:
$\textsc{RegisterAuditor}$ and $\textsc{Audit}$. A new ``analyst'' party
$\enanalyst$ can be registered as authorised to compute function $\enanalfunc$
over all secret inputs uploaded by infected users (in what we call an ``audit'' procedure).
An auditor is allowed to register a function only if it belongs to
the set of allowable functions $\enanalfuncset$ (discussed below). While the
ideal functionality simply evaluates the specific audit function over the
appropriate physical reality fields, to implement this new feature we rely on
the FESR primitive as a subroutine. In particular, we rely on the notion of
Functional Encryption as an access-controlled repository (introduced in
\cite{DBLP:conf/csfw/0002M15}) to replace the Trusted Bullettin Board. Users who
desire to share their exposure can now call onto FESR's encrypt procedure, which
essentially uploads some data to an ideal trusted repository. All protocol
users, on setup, are authorised (i.e. they receive a FESR functional key) to
decrypt the $\mathsf{risk}$ function, which simply returns the list of protocols
infected in the last $\incubt$ days (the period of incubation for the disease),
so that the user can estimate their risk factor locally. Auditor parties instead
are authorised to compute any function for which they successfully run a
$\textsc{RegisterAuditor}$ call. The function is evaluated directly by the FESR
ideal machine, and the auditor simply receives the return value, without
learning anything about the function inputs.

\begin{functionality}{$\phyidealfunc$ sketch}
 \textsc{input}: the \textsf{MeasurableRealityRecord} data structure can now mark some records with label $\phyrecsec$

 \textsc{MyCurrentMeas}: only returns non-$\phyrecsec$ fields from the user record

 Otherwise, proceeds as in original
\end{functionality}

\begin{functionality}{$\enidealfunc$ sketch}
  \begin{receive}[\enanalyst]{RegisterAuditor}{\enanalfunc}
    \State record $\enanalyst$ as capable of decrypting function $\enanalfunc$ over ciphertexts
  \end{receive}

  \begin{receive}{Audit}{\enanalfunc}
    \If{$(\party,\enanalfunc)$ are registered}
    \State get noisy record from physical reality functionality
    \State evaluate $\enanalfunc$ over physical reality noisy record $\phyrecsec$ fields (outputs y)
    \State \Send{Audit}{\party,\enanalfunc,y}{\adversary}
    \State \Return y
    \EndIf
  \end{receive}

  Other function calls proceed as in the original paper
\end{functionality}

\begin{protocol}{$\protoname$}
\label{proto:proto}
  \begin{receive}[\environment]{ActivateMobileUser}{\enuser}
    \State ask C to \Send{setup}{\enuser}{\fesr}
    \State ask C to \Send{keygen}{\mathsf{risk},\enuser}{\fesr}
  \end{receive}
  \begin{receive}{RegisterAuditor}{\enanalyst,\enanalfunc}
    \State ask C \Send{keygen}{\enanalyst,\enanalfunc}{\fesr}
    \State mark $(\party,\enanalfunc)$ as registered
  \end{receive}
  \begin{receive}{ShareExposure}{}
    \State check exposure status with $\phyidealfunc$
    \If{positive}
    \Send{Encrypt}{SentChirps; SensorData}{\fesr}
    \EndIf
  \end{receive}
  \begin{receive}{ExposureCheck}{}
    \State \SendAndReceive{Decrypt}{\mathsf{risk}}{\fesr}{list}
    \State check list for any matches with local list of received chirps
  \end{receive}

  \begin{receive}{Audit}{\enanalfunc}
    \If{$(\party,\enanalfunc)$ are registered}
    \State \SendAndReceive{Decrypt}{\enanalfunc}{\fesr}{y}
    \Return $y$
    \EndIf
  \end{receive}

  Other function calls proceed as in the original paper
\end{protocol}

Our simulation strategy is similar to that of
\cite{EPRINT:CKLRSSTVW20}. For all operations that relate
strictly to the exposure notification portion of the ideal functionality, we
simply run the same operation as Canetti's simulator. We also augment some new and
existing procedure with our own simulator code, as follows
\begin{simulator}{Sim sketch}
  \item \textbf{ShareExposure}: to accommodate our additional features, our
  version of the ShareExposure procedure needs to allow both the upload of the
  normal Rebabbler chirps, as well as our new $\phyrecsec$ data. In the honest
  user case, the ideal procedure is equivalent to the protocol; % is this true?
  For the \textbf{AdvUpload} case, we first check that the corrupted party was
  infected (still relying on a Canetti assumption, it might be nice to add some
  authentication from a testing facility). Next, the simulator applies a fake
  reality function to the physical reality functionality, such that the reality
  store now includes the modified adversarial input. As long as the adversarial
  input is physically sensible (i.e. can realistically happen in physical
  reality), the PhyReal functionality should accept this modification. With a
  modified physical reality, we call the ShareExposure Ideal
  functionality. % we need to argue that there exist an appropriate forgery function

  \item \textbf{ExposureCheck} proceeds as in Canetti, ignoring the $\phyrecsec$ field
  \item \textbf{RegisterAuditor} simply calls the ideal RegisterAuditor; might need to simualte network traffic between KeyManagement party and Auditor
  \item \textbf{Audit/Decrypt (FESR)}: The simulator has to keep synchronised the Real World function state in FESR with the decryptions returned by the Ideal Audit function; thus on any call to either the Audit procedure of EN or the decrypt procedure in FESR, the corresponding procedure on the other functionality is also called with the appropriate argument.  % we need to specifiy how each argument is obtained by the adversarial party
% e.g. The Leakage function is extended to return the FESR indexes for uploaded ciphertexts, so that the simulator can synchronise calls between ...
  \item \textbf{Corrupt}: to preserve post-compromise security (and avoid deniability issues), we assume that on corruption, all user data is wiped
  \item \textbf{RecordMeas}: Proceeds as in Canetti, but can store both normal and secret data
  \item \textbf{ReportState}: proceeds as in Canetti, without returning the secret data
  \item \textbf{SetAntennaSensitivity}: records the adversarial parameters for Bluetooth antenna sensitivity, and any other sensors; can be used by the fake reality functionalities
  \item \textbf{AdvChirp}: should be unchanged from Canetti, as chirps do not include any information about our additional inputs
\end{simulator}

TODO Key Management party

\subsubsection{Allowable functions}
FESR allows us to have stateful and non-deterministic programs
TODO discuss - privacy implications?
\subsection{UC}
\subsubsection{FESR}
The Functional Encryption for Stateful and Randomised functions ($\fesr$)
primitive was introduced by \cite{PKC:BKMT21}, where it was shown that it can be
implemented through a simple protocol using Trusted Execution Environments in a
UC-secure manner. We reproduce the original FESR functionality in section
\ref{sec:fesr}. To realise the protocol described in figure \ref{proto:proto},
we have to slightly modify this. The original $\fesr$ produces a handle when
encrypting, (effectively an idealised representation of the ciphertext), and
separates the state of each function between decryptors (i.e. given two
decryptors Alice and Bob authorised to compute some function $\funcF$, only
Decryption calls for $\funcF$ initiated by Alice affects Alice's state, regardless of any
calls Bob might make). The functionality in our protocol behaves slightly
differently: we are not particularly interested in the users storing individual
handles for their encrypted text, as we want decryption calls to be computed
over all uploaded data from all users. Additionally, some functionalities might
require to share state among auditors. It is straightforward to use the existing
$\fesr$ functionality to create a new $\fesr'$ that implements these features.

To realise $\fesr'$, we instantiate a single-decryptor $\fesr$. The $\fesr'$ protocol proceeds as follow
\newcommand{\funcMerge}{\mathsf{merge}}
\newcommand{\funcFplusMerge}{\funcF \circ \funcMerge}
\newcommand{\inputskw}{\mathsf{inputs}}
\newcommand{\statekw}{\mathsf{state}}
\begin{protocol}{$\fesr'[\fesr]$}
  \begin{receive}[none]{setup}{\party}
    \State same as in $\fesr$
  \end{receive}
  \begin{receive}[\PartyC]{keygen}{\funcF}
    \State\Send{keygen}{\PartyB,\funcFplusMerge}{\fesr}
  \end{receive}
  \begin{receive}[\party \in \{\PartyA,\PartyB\}]{encrypt}{x}
    \State \SendAndReceive{encrypt}{\fein}{\fesr}{\handle}
    \State \SendAndReceive{decrypt}{\handle}{\funcFplusMerge}{\epsilon}
  \end{receive}
  \begin{receive}[\PartyB]{decrypt}{\funcF}
    \State\SendAndReceive{decrypt}{\epsilon,\funcFplusMerge}{\fesr}{\feout}
    % nope
  \end{receive}
  \begin{algorithmic}
    \State def \underline{$\funcFplusMerge(\fein,\festate):$}
    \If{$\fein \neq \epsilon$}
      \State$\festate[\inputskw]\gets\festate[\inputskw] \concat \fein;\feout\gets\epsilon$
    \Else
      \State$(\feout, \festate') \gets \funcF(\festate[\inputskw],\festate[\statekw])$
      \State$\festate[\statekw] \gets \festate'$
    \EndIf
    \State\Return($\feout,\festate$)
  \end{algorithmic}
\end{protocol}

The above protocol is a simple wrapper around the original $\fesr$ functionality, which abstracts away from the use of handles and allows evaluating functions over all concatenated inputs. To sidestep the restrictions of $\fesr$, we define a new stateful function $\funcFplusMerge$, which allows us to both concatenate the inputs (stored in $\festate[\inputskw]$) and to compute stateful function $\funcF$ (whose state is kept in $\festate[\statekw]$).

TODO: proof?

The above steps could also be explicitly incorporated as part of our protocol while communicating with the original $\fesr$, but we abstract this type of communication for simplicity.

TODO (CrowdNotifier): extend FESR to have multiple keygen authorities, to decentralise keygen
One common criticism of Functional Encryption is that it promotes centralisation, by giving power to the Trusted Authority to generate secret keys. If the Trusted Authority decides to collude with a Decryptor, they are able to reveal the original inputs to a ciphertext. The $\fesr$ identifies the trusted authority as $\PartyC$, and while the $Steel$ protocol assumes the presence of a single instance of $\PartyC$, the functionality does not exclude that there might be multiple $\PartyC$ parties (corresponding to the notion of Multiple Authority Functional Encryption).
(another potential idea is that of decentralised or ad-hoc FE and their generalisation of Dynamic Decentralised Functional Encryption to let the set of users generate keygen - removes trust from trusted authority; alternatively, Delegatable FE allows keygen to be hierarchical for ``increasingly restrictive'' function authorisations)

TODO Define Post compromise security
\subsubsection{Proof (sketch?)}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> extensions.tex <==
\section{Extensions}
\subsection{Active adversary}
Server can affect the heatmap

problems: how do we get server not to input fake data? {signed by certifier, add noise}
\subsection{Collusion}
\subsection{Verifiability}
We want to make sure the server returns the correct map it generated;
\section{...}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> functionality.tex <==
\paragraph{Outline}
We describe a protocol that augments a decentralised contact tracing scheme to add a confidential auditing functionality.
The protocol involves a series of clients (most likely mobile devices or hardware tokens) - the users; a central Bulletin board, which is publicly accessible, and a set of parties who are interested in analysing information about the disease spread - the auditors.
A user, while the contact tracing program is active on their device, records two sets of information: a ``public'' value, which can be safely shared unencrypted as it doesn't reveal any personally identifiable information, and a ``secret'' value which requires encryption when  uploaded to the public repository (i.e. the user's geolocation). After a client is activated, they begin broadcasting chirps, based on their current public measurements (e.g. time) and a freshly sampled seed, which are immediately erased. At the same time, the user listens for incoming transmissions, and stores any chirp received. Chirps older than the incubation period for the disease are erased.
When a user is diagnosed as infected (outside the scope of the protocol), they will Share their Exposure status with a central Bulletin, Board. To do this, the user uploads the list of generated chirps, and (encrypted) secret data to a public bulletin board, and stops broadcasting.
Any active user can check their infectious status by downloading the set of public data from the Bulletin Board. If any of the chirps uploaded within the incubation period match with any of their locally heard chirps, they can be considered infectious and should self-isolate.
An \textit{auditor} can request the protocol for permission to compute a function based on the secret data uploaded by exposed users. A trusted third party can generate a Stateful and Randomised Functional Encryption (FESR)
functional key to grant auditors permission to compute a certain function; this
allows the auditors to evaluate the function over all upload user secret data, without learning its original plaintext values.


\paragraph{Notation}
\begin{itemize}
  \item function $\mathsf{map}(F,A)$ returns the list containing the application of function $F$ to all elements of list A
  \item A[B] indicates accessing the field labelled B within array A; if B is a list, it returns a list containing all entries in A matching with labels in B; allows chaining to access nested objects (A[B][C])
  \item $A \stackrel{?}{\in} B$ is the boolean function that returns true if object A is part of data structure B, false otherwise
\end{itemize}

% verify: if !condition , halt

The Physical reality functionality stores a list of record for each user that submitted one.
Records contain both a public and private portion.
Known record times are
\begin{itemize}
  \item $\phyrectime$ - time of production of the current record
  \item $\phyrecdist[\enuser]$  records the distance of the current user from $\enuser$  in meters
  \item $\phyrectrpw$ - transmission power for the current user
\end{itemize}

We augment the original $\phyidealfunc$ with an additional well-formedness predicate $\phywellfpred$ and split the user inputs in a public $\phyusermeas$ and secret $\phyusersec$ value.
The real world validity predicate $\phyvalpred$ still operates on all public inputs provided by (possibly corrupted users), and $\phywellfpred$ verifies the well-formedness of secrets. When accessing user records, the $\phyrecfields$ values can only include the public inputs, but priviliged parties in $\phyprivents$  also receive the private inputs

\begin{functionality}{$\phyidealfunc[\phyvalpred,\phywellfpred,\phyprivents]$}
  \begin{receive}{Setup}{}
    \State $\phymeasrec \gets \emptyset$
  \end{receive}
  \begin{receive}{input}{\enuser,\phyusermeas,\phyusersec}
    \State $\phymeasrec[\enuser] \gets \phymeasrec[\enuser] \concat \{\phyusermeas,\phyrecsec: \phyusersec\}$
    \State \SendAndReceive{time}{}{\timeidealfunc}{\timecntr}
    \State verify $\timecntr = \phyusermeas[\phyrectime] \land \phyvalpred(\phymeasrec) \land \phywellfpred(\phymeasrec)$
  \end{receive}
  \begin{receive}{MyCurrentMeas}{\enuser,\phyrecfields,\phyerrfunc}
    \If{$\party \not\in \{\enuser,\phyprivents\}$}  % \lor (\party = \enuser \land \phyrecsec \in \phyrecfields)}
      \Return error
    \Else
      \State $\phyusermeas \gets \phymeasrec[\enuser][-1]$
      \State \Return $\phyerrfunc(\phyusermeas[\phyrecfields])$
    \EndIf
  \end{receive}
  \begin{receive}[\mathit{F} \in \phyprivents]{AllMeas}{\phyerrfunc}
    \State $\widetilde{\phymeasrec} \gets \mathsf{map}(\phyerrfunc,\phymeasrec)$
    \State \Return $\widetilde{\phymeasrec}$
  \end{receive}
\end{functionality}

\begin{functionality}{$\timeidealfunc$}
  \begin{statedecl}
    \statevar{\timecntr}{0}{Elapsed time counter}
  \end{statedecl}
  \begin{receive}[\environment]{increment}{}
    \State $\timecntr \gets \timecntr + 1$
  \end{receive}
  \begin{receive}{time}{}
    \State \Return $\timecntr$
  \end{receive}
\end{functionality}

The $\enidealfunc$ augments the original formulation with two additional procedures: $\textsc{RegisterAuditor}$ allows the environment to authorise a new party to compute a function of type $\enanalfuncset$ on the secret input for all users who have shared their exposure status; $\textsc{Audit}$ allows one such party to receive the result for a function they have been authorised to compute. Since the $\ennoisyrec$ now holds secret input from all users, the $\enleakfunc$ needs to accurately portray the amount of leakage for the secret information as well, taking into account that (in a real world protocol) secrets for users who haven't shared their exposure are still kept on the client, and for those that have the secret will be likey encrypted (so only metadata such as ciphertext length would be leaked).
\begin{functionality}{$\enidealfunc[\enriskfunc,\enerrorfuncset,\enfakingfuncset,\enleakfunc,\enanalfuncset]$}
  \begin{statedecl}
    \statevar{\ennoisyrec}{}{Noisy record of physical reality}
    \statevar{\ensharexprec}{}{List of users who have shared their exposure status}
    \statevar{\enusers}{}{List of active users}
    \statevar{\enuserscorr}{}{List of corrupted users}
    \statevar{\enanalfuncset}{\enanaldomain \rightarrow \enanalrange}{Function class for analysis functions}
    \statevar{\enanalysts}{}{List of authorised analysts and their functions of type $\enanalfuncset$}
  \end{statedecl}
  \begin{receive}[\simul]{Setup}{\epsilon^{*}}
    \State verify $\epsilon^{*} \in \enerrorfuncset$
    \State $\ennoisyrec \gets \emptyset$
  \end{receive}
  \begin{receive}{ActivateUser}{\enuser}
    \State $\enusers \gets \enusers \concat \enuser$
    \State \Send{ActivateUser}{\enuser}{\simul}
  \end{receive}
  \begin{receive}{RegisterAuditor}{\enanalyst,\enanalfunc}
    \If{$\enanalfunc \in \enanalfuncset$}
      \State $\enanalysts \gets \enanalysts \concat (\enanalyst, \enanalfunc)$
    \EndIf
    \State \Send{RegisterAuditor}{\enanalyst,\enanalfunc}{\simul}
  \end{receive}
  \begin{receive}{ShareExposure}{\enuser}
    \State \SendAndReceive{AllMeas}{\epsilon^{*}}{\phyidealfunc}{\ennewnoisyrec}
    \State $\ennoisyrec \gets \ennoisyrec \concat \ennewnoisyrec$ % maybe we need to use set union here?
    \State $\mu \gets \ennoisyrec[\enuser] \concat \ennoisyrec[\ensharexprec]$
    \If{$\ennoisyrec[\enuser][\phyrecinf] = \bot$}
    \State \Return
    \Else
      % \If{$\enuser \in \enuserscorr$}
        % \State $\ensharexprec \gets \ensharexprec \concat \enuser$
        % double check this: no time inserted, keeps in active users

      \State \SendAndReceive{time}{}{\timeidealfunc}{\mathit{t}}
      \State $\ensharexprec \gets \ensharexprec \concat (\enuser,\mathit{t})$
      \State $\enusers \gets \enusers \setminus \{\enuser\}$
      \If{$\enuser \in \enuserscorr$}
      \State \Send{ShareExposure}{}{\simul}
      \EndIf
    \EndIf
  \end{receive}
  \begin{receive}{ExposureCheck}{\enuser}
    \If{$\enuser \not\in \enusers$}
      \Return error
    \Else
    \State \SendAndReceive{AllMeas}{\epsilon^{*}}{\phyidealfunc}{\ennewnoisyrec}
    \State $\ennoisyrec \gets \ennoisyrec \concat \ennewnoisyrec$ % maybe we need to use set union here?
    \State $\mu \gets \ennoisyrec[\enuser] \concat \ennoisyrec[\ensharexprec]$
      \State \Return $\enriskfunc(\enuser,\mu)$
    \EndIf
  \end{receive}
  \begin{receive}{RemoveMobileUser}{\enuser}
      \State $\enusers \gets \enusers \setminus \{\enuser\}$
  \end{receive}
  \begin{receive}{Audit}{\enanalfunc}
    \If{$(\party,\enanalfunc) \in \enanalysts$}
      \State $y \gets \enanalfunc(\ennoisyrec[\ensharexprec][\phyrecsec])$
      \Send{Audit}{\enanalfunc,\party,y}{\adversary}
      \State \Return $y$
    \EndIf
  \end{receive}
  \begin{receive}[\simul]{Corrupt}{\enuser}
    \State $\enuserscorr \gets \enuserscorr \concat \enuser$
  \end{receive}
  \begin{receive}[\simul]{MyCurrentMeas}{\enuser,\phyrecfields,\phyerrfunc}
    \If{$\enuser \in \enuserscorr$}
    \State \SendAndReceive{MyCurrentMeas}{\enuser,\phyrecfields,\phyerrfunc}{\phyidealfunc}{\phymeasret}
    \State \Send{MyCurrentMeas}{\phymeasret}{\simul}
    \EndIf
  \end{receive}
  \begin{receive}[\simul]{FakeReality}{\phi}
    \If{$\phi \in \enfakingfuncset$}
      \State $\ennoisyrec \gets \phi(\ennoisyrec)$
    \EndIf
  \end{receive}
  \begin{receive}[\simul]{Leak}{}
    \State \Send{Leak}{\enleakfunc(\{\ennoisyrec, \enusers, \ensharexprec\})}{\simul}
  \end{receive}
  \begin{receive}[\environment]{IsCorrupt}{\enuser}
    \State \Return $\enuser \stackrel{?}{\in} \enuserscorr$
  \end{receive}
\end{functionality}


\paragraph{Protocol}
\begin{functionality}{$\btidealfunc$}
  \begin{statedecl}
    \statevar{\btmesrec}{}{Records BT measurements sent by users}
  \end{statedecl}
  \begin{receive}[\enuser]{BTListen}{\btantstr,\btrecfields,\bterrfunc}
    \State $\btmesrec[\enuser] \gets (\btantstr,\btrecfields,\bterrfunc)$
  \end{receive}
  \begin{receive}[\enuser]{BTSend}{\btmsg,\bttp}
    \State \SendAndReceive{AllMeas}{\bot}{\phyidealfunc}{\phymeasrec}
     \Comment{$\bot$ here corresponds to the identity function}
     \For{$\enuser' \in \phymeasrec$}
      \State \SendAndReceive{time}{}{\timeidealfunc}{\mathit{t}}
     \State $\btdis{\enuser}{\enuser'} \gets (\{\phyrecdist[\enuser'],\phyrectime = t\} \in \phymeasrec[\enuser])$
     \If{$\btdis{\enuser}{\enuser'} \leq \phymeasrec[\enuser'][\phyrectrpw] \times \delta \times \bttp$}
    \State $\btatt \gets \bterrfunc(\btdis{\enuser}{\enuser'})$
    \State \SendAndReceive{MyCurrentMeas}{\enuser,\btrecfields,\bterrfunc}{\phyidealfunc}{\phymeasret}
    \State $\btrec \gets \btrec \concat (\enuser',\btmsg,\phymeasret,\btatt)$
    \EndIf
    \EndFor
  \end{receive}
  \begin{receive}[\enuser]{BTReceive}{}
    \State \Return $\btrec[\enuser,\cdot,\cdot,\cdot]$
  \end{receive}
\end{functionality}

% \begin{functionality}{$\tbbidealfunc[\enscheme]$}
%   \begin{statedecl}
%     \statevar{\tbbrec}{}{Record for uploaded data}
%     \statevar{\tbbsecrec}{}{Record for uploaded secret data}
%   \end{statedecl}
%   \begin{receive}[\enuser]{Add}{\tbbin,\tbbsecin}
%     \Comment{Should first check that U is infectious through $\phyidealfunc$ }
%     % \State \SendAndReceive{AllMeas}{\bot}{\phyidealfunc}{\phymeasrec}
%     % if true
%     \State $\tbbrec \gets \enscheme.\enmerge(\tbbrec,\tbbin)$
%     \State $\tbbsecrec \gets \tbbsecrec \concat \tbbsecin$
%   \end{receive}
%   \begin{receive}[\enuser]{Retrieve}{}
%     \State \Return $\tbbrec,\tbbsecrec$
%   \end{receive}
% \end{functionality}
\newcommand{\Fmerge}{\mathsf{merge}}
\newcommand{\Frisk}{\mathsf{risk}}
We say that $\fesr's \Ffamily = \{\Fmerge,\Frisk\} \cup \enanalfuncset$ where
$\Fmerge(x,s) := (\empty,s \concat x)$,
$\Frisk(\empty,s) := (\empty,s[*,\bot])$

\begin{protocol}{$\protoname[\enscheme,\phyrecfields^*,\phyerrfunc,\bttp,\btantstr,\protottl,\protopp,\enanalfuncset]$}
  \begin{statedecl}
    \statevar{\enuserscorr}{}{List of corrupted users}
    \statevar{\enanalfuncset}{\enanaldomain \rightarrow \enanalrange}{Function class for analysis functions}
    \statevar{\enanalysts}{}{List of authorised analysts and their functions of type $\enanalfuncset$}
  \end{statedecl}
  \begin{receive}{ActivateMobileUser}{\enuser}
    \State $(\protostsent,\protostrec) \gets \emptyset$
    \State \Send{Setup}{\enuser}{\fesr} through $\PartyC$
    \State \SendAndReceive{keygen}{\Fmerge}{\fesr}{\msg{Assigned}{\fesr}} through $\PartyC$
    \State \Send{BTListen}{\enuser,\btantstr,\phyrecfields^{*},\phyerrfunc}{\btidealfunc}
    \State $t' \gets 0$
    \Comment{we should call input on $\phyidealfunc$}
    \State $\protochrpng = \top$
    \While{$\protochrpng = \top$}
    % really until we receive the removemobileuser message
      \Comment{Start Chirping:}
      \State \SendAndReceive{Time}{}{\timeidealfunc}{\timecntr}
      \If{$\timecntr - \protolasttime \leq \protottl$}
        \State \SendAndReceive{MyCurrentMeas}{\enuser,\phyrecfields^{*},\phyerrfunc}{\phyidealfunc}{\protomeas}
        \State $\protosec \gets \enscheme.\enkeygen(\protopp)$
        \State $\protochirp \gets \enscheme.\enchirp(\protosec,\protomeas)$
        \State \Send{BTSend}{\protochirp,\bttp}{\btidealfunc}
        \State securely erase $\protosec,\protochirp$
      \EndIf
      \Comment{Listen:}
      \State \SendAndReceive{BTReceive}{}{\btidealfunc}{\protobtrec}
      \State $\protostrec[\timecntr] \gets \protobtrec$
      \Comment{Zero all the data collected before the infection window $\protottl$}
      \State $\protostsent[\cdot \leq \timecntr - \protottl] \gets \emptyset$
      \State $\protolasttime \gets \timecntr$
    \EndWhile
  \end{receive}
  \begin{receive}[\environment]{RegisterAuditor}{\enanalyst,\enanalfunc}
    \Comment{the protocol acts as the $\fesr$ party C}
    \If{$\enanalyst \not\in\enanalysts$}
      \State \Send{Setup}{\enanalyst}{\fesr} through $\PartyC$
      \State $\enanalysts[\enanalyst] \gets []$
    \EndIf

    \If{$\enanalfunc \in \enanalfuncset$}
      \State \Send{Keygen}{\enanalfunc,\enanalyst}{\fesr}
      \State $\enanalysts[\enanalyst] \gets \enanalysts[\enanalyst] \concat \enanalfunc$
    \EndIf
  \end{receive}
  \begin{receive}{Audit}{\enanalfunc,input}
    \If{$(\party,\enanalfunc) \in \enanalysts$}
      \State \SendAndReceive{Decrypt}{input}{\fesr}{\msg{Decrypted}{y}}
    \EndIf
  \end{receive}
  \begin{receive}{ShareExposure}{\enuser}
    \State \SendAndReceive{MyCurrentMeas}{\enuser,\phyrecinf,\identityfunc}{\phyidealfunc}{\protomeas}
    \If{$\protomeas = true$}
      \State \SendAndReceive{MyCurrentMeas}{\enuser,\phyrecsec,?}{\phyidealfunc}{\protomeas_{sec}}
      \State $\protodb \gets \enscheme.\enupload(\protostsent,\protostrec \concat ct)$
      \State \SendAndReceive{encrypt}{\protodb}{\fesr}{\handle}
      \State \SendAndReceive{encrypt}{\protomeas_{sec}}{\fesr}{\handle'}  % sent as A
      \State \SendAndReceive{decrypt}{(\handle,\bot),\Fmerge}{\fesr}{\empty}
      \State \SendAndReceive{decrypt}{(\handle',\top),\Fmerge}{\fesr}{\empty}
      \State securely erase all state
    \EndIf
  \end{receive}
  \begin{receive}{ExposureCheck}{\enuser}
    \State \SendAndReceive{Decrypt}{h0,\Fmerge}{\fesr}{\tbbrec}
    \State  $\protoriskscore \gets \enscheme.\encheck(\protosec,\protostrec,\tbbrec)$
    \State \Return $\protoriskscore$
  \end{receive}
  \begin{receive}{RemoveMobileUser}{\enuser}
    \State securely erase $\protostsent,\protostrec$
    \State $\protochrpng \gets \bot$
  \end{receive}
  % adv
  \begin{receive}{Corrupt}{\enuser}
    \State $\enuserscorr \gets \enuserscorr \concat \enuser$
  \end{receive}
  \begin{receive}{RecordMeas}{\enuser,\phyrecfields}
    \If{$\enuser \in \enuserscorr$}
    \State \SendAndReceive{MyCurrentMeas}{\enuser,\phyrecfields,\identityfunc}{\phyidealfunc}{\protomeas}
    \State \Return $\protomeas$
    \EndIf
  \end{receive}
  \begin{receive}{ReportState}{\enuser}
    \If{$\enuser \in \enuserscorr$}
    \State \SendAndReceive{BTReceive}{\enuser}{\btidealfunc}{\protomeas}
    \State $\protostrec \gets \protostrec \concat \protomeas$
    \State \Return ($\protostrec, \protostsent$)
    % TODO: should receive list of ctxts?
    \EndIf
  \end{receive}
  \begin{receive}{SetAntennaSensitivity}{\enuser,\btantstr,\phyrecfields,\phyerrfunc}
    \If{$\enuser \in \enuserscorr$}
    \State \Send{BTListen}{\btantstr,\phyrecfields,\phyerrfunc}{\btidealfunc}
    \EndIf
  \end{receive}
  \begin{receive}{AdvChirp}{\enuser,\btantstr,p}
    \If{$\enuser \in \enuserscorr$}
    \State \Send{BTSend}{\btantstr,p}{\btidealfunc}
    \EndIf
  \end{receive}
  \begin{receive}{AdvUpload}{a}
    \If{$\enuser \in \enuserscorr$}
    \State \Send{Add}{a}{\tbbidealfunc}
    \EndIf
  \end{receive}
  \begin{receive}[\environment]{IsCorrupt}{\enuser}
    \State \Return $\enuser \stackrel{?}{\in} \enuserscorr$
  \end{receive}

\end{protocol}
\paragraph{Simulator}
\newcommand{\leaklcor}{L_{\mathsf{cor}}}
\newcommand{\leaklup}{L_{\mathsf{up}}}
\newcommand{\leaklsec}{L_{\mathsf{sec}}}
\newcommand{\leakneigh}{N_{\enuser,t}}
\newcommand{\btboosting}{\beta}
\newcommand{\simulincub}{\tau}
\newcommand{\simulchirpint}{\mathit{I}}
\newcommand{\simulinfd}{d_\mathit{I}}
\newcommand{\simullocseeds}{\mathit{C}}
\newcommand{\simulupseeds}{\mathit{\widetilde{C}}}
\newcommand{\simulchirps}{\mathit{D}}
\newcommand{\simulantennas}{\overline{As}}

\begin{algorithmic}
 % \State \Underline{Leakage function}
 \Procedure{$\enleakfunc_{r^{*}}$}{$\enstate$}
 \State parse $(\phymeasrec,\ensharexprec) \gets \enstate$
 \State $\leaklcor \gets []$
 \State $idsarray \gets []$
 \For{time unit $t$}
 \For{$\enuser \in \enusers$}   % these should be the active users at time t
   \State $idsarray \gets (\enuser,t)$
   \State $\protomeas \gets \phymeasrec[\enuser][\protomeas,t]$
   \State $\hat{U} \gets \enuser \stackrel{?}{\in} \enuserscorr$
   \If{$\enuser$ was corrupted at time t}
   \State $r_{\enuser,\enuser'} \gets r^{*}$
   \Else
   \State $\btboosting_{\enuser'} \gets$ boosting signal, set by simulator (somehow)
   \State $r_{\enuser,\enuser'} \gets r^{*} \times \btboosting_{\enuser'}$
   \EndIf
   \State $N_{\enuser,t} \gets {\enuser' : \phymeasrec[\enuser][\phyrecdist[\enuser',t]] < r_{\enuser,\enuser'} \land \phymeasrec[\enuser'][corrupt]} $
   \State $\leaklcor \gets (\protomeas,\hat{U},N_{\enuser,t})$
 \EndFor
 \EndFor
 \For{$i \in \ensharexprec$}
   \State $(\enuser_{k_{i}},t_{i}) \gets \ensharexprec[i]$
   \State $j \gets FindIndex((\enuser_{k_{i}},t_{i}),idsarray)$
   \State $\leaklup \gets \leaklup \concat (i,j)$
  \EndFor
 \State $\leaklsec \gets ...$
 \State \Return $(\leaklcor,\leaklup,\leaklsec)$
 \EndProcedure
\end{algorithmic}

 % reality faking function
\begin{simulator}{S[$\simulincub,\simulchirpint$]}
  \begin{statedecl}
    \statevar{\simullocseeds}{}{List of locally stored seeds per-user}
    \statevar{\simulupseeds}{}{List of simulated seeds uploaded to $\tbbidealfunc$}
    \statevar{\simulchirps}{}{List of simulated chirps $(j,\protosec,\protomeas,\protochirp)$}
    \statevar{\enuserscorr}{}{List of corrupted users}
    \statevar{\ensharexprec}{}{List of users who have shared their exposures}
    \statevar{\simulantennas}{}{Bluetooth antenna sensitivity values}
  \end{statedecl}
  \begin{receive}[\environment]{Corrupt}{\enuser}
    \State \Send{Corrupt}{\enuser}{\enidealfunc}
    \State $\enuserscorr \gets \enuserscorr \concat \enuser$
  \end{receive}
  \begin{receive}[\environment]{RecordMeas}{\enuser,\phyrecfields}
    \If{$\enuser \in \enuserscorr$}
    \State \Send{MyCurrentMeas}{\enuser,\phyrecfields}{\enidealfunc}{out}
    \State \Return out
    \EndIf
  \end{receive}
  \begin{receive}[\environment]{ReportState}{\enuser}
    \State \SendAndReceive{Leak}{\enleakfunc}{\enidealfunc}{(\leaklcor,\leaklup)}
    \Comment{Stored seeds:}
    \If{$\enuser \in \ensharexprec$}
      \State \Return $\epsilon$
    \Else
      \For{$(\protomeas,\enuser,\leakneigh) \in \leaklcor$}
        \If{$(j,\protosec,\protomeas,\protochirp) \not\in \simulchirps$}
          \State $\protosec \samuni \seedrange$
          \State $\simulchirps \gets \simulchirps \concat (j,\protosec,\protomeas,\enscheme.\enchirp(\protosec,\protomeas))$
        \EndIf
        \State $\simullocseeds \gets \simullocseeds \concat  \protosec$
      \EndFor
    \EndIf
    \Comment{Recorded Chirps:}
    \State $\protostrec \gets \emptyset$
    \For{$j \in \leaklcor$}
      \State $(\protomeas,\enuser',N) \gets \leaklcor[j]$
      \If{$\enuser \in N$}
        \If{$(j,\protosec,\protomeas,\protochirp) \not\in \simulchirps$}
          \State $\protosec \samuni \seedrange$
          \State $\simulchirps \gets \simulchirps \concat (j,\protosec,\protomeas,\enscheme.\enchirp(\protosec,\protomeas))$
        \EndIf
        \State $\protomeas \gets \protomeas \concat (\protochirp,\protomeas)$
      \EndIf
    \EndFor
    \State $\ensharexprec \gets \ensharexprec \concat \enuser$
  \end{receive}
  \begin{receive}[\environment]{Retrieve}{\enuser}
    \If{$\enuser \in \enuserscorr$}
      \State \Return $\simulupseeds$
    \EndIf
  \end{receive}
  \begin{receive}[\environment]{AdvChirp}{\enuser,a,p}
    \Comment{$a \in \seedrange$}
    \State \SendAndReceive{Leak}{\enleakfunc}{\enidealfunc}{(\leaklcor,\leaklup,\_)}
    \Comment{Fetch latest entry in $\leaklcor$ for current user}
    \State $\ell_{j} \gets \leaklcor[\cdot,\enuser,\cdot][-1]$
    \State $\simulchirps \gets \simulchirps \concat (j,\bot,\protomeas,a)$
    \For{$(j',\protosec',\protomeas',\protochirp) \in \simulchirps,\protomeas' = \protomeas,\protochirp=a$}
      \State $(\protomeas',\enuser',N') \gets \leaklcor[j]$
      \State $\phi \gets \lambda(\phymeasrec): \{$
        \State $\widetilde{N} \gets [\enuser': \{\phyrecdist[\enuser']=d\delta \times \bttp$ % TODO syntax, as corrupt?
        \For{$\enuser'' \in \widetilde{N}$}
          \State $\enuser'  \gets \leaklcor[j'][1]$
          % \note{This is bot when the user is not corrupt}
          \State $d'' \gets d(\enuser,\enuser'')$
          \If{$\enuser'$ is corrupted at time of transmission}
          $p' \gets \phymeasrec[\enuser'][tp]$
          \Else{} $p' \gets tp_{0}$
          \EndIf
          \State $d' \gets d'' \cdot p'/p$
          \State $\phymeasrec[\enuser''] \gets (d',\enuser')$
        \EndFor
      $\}$
      \State \Send{FakeReality}{\phi}{\enidealfunc}
    \EndFor
    \State \Return
  \end{receive}
  \begin{receive}[\environment]{AdvUpload}{\enuser,\simullocseeds}
    \State \Assert $\enuser \in \enuserscorr$
    \State \SendAndReceive{Leak}{\enleakfunc}{\enidealfunc}{(\leaklcor,\leaklup)}
    \State \Assert  $\enuser$ is infected
    \Comment{Remove $\enuser$ from unreported encounters}
    \For{$\ell_{j} = (\protomeas,\enuser,\leakneigh) \in \leaklcor$}
      \State find $(j,\protosec,\protomeas,\protochirp)$
      \If{$\protosec \not\in \simullocseeds$}
        \State $\phi \gets \lambda(\phymeasrec): \{$
          \For{$\enuser' \in \leakneigh$}
            \State $\phymeasrec[\enuser'][d_{\enuser,t}] \gets \simulinfd + R$ % TODO: syntax
          \EndFor
        $\}$
        \State \Send{FakeReality}{\phi}{\enidealfunc}
      \EndIf
    \EndFor
    \Comment{Add $\enuser$ to encounters of other corrupted users}
    \For{$\protosec \in \simullocseeds$}
      \For{$(j,\protosec',\protomeas,\protochirp)$}
        \If{$(s' = s \lor s' = \bot) \land \protochirp = \enscheme.\enchirp(\protosec,\protomeas)$}
          \State $(\protomeas,\hat{\enuser}',N_{\enuser',t}) \gets \leaklcor[j]$
          \State $\phi \gets \lambda(\phymeasrec): \{$
            \For{$\enuser'' \in N_{\enuser',t}$}
              \State $d_{\enuser,\enuser'',t} \gets d_{\enuser',\enuser'',t} $ % TODO get proper fields
            \EndFor
          $\} $
          \State \Send{FakeReality}{\phi}{\enidealfunc}
        \EndIf
      \EndFor
    \EndFor
    \Send{ShareExposure}{\enuser}{\enidealfunc}
  \end{receive}
  \begin{receive}[\environment]{SetAntennaSensitivity}{\enuser,\btantstr,\phyrecfields,\phyerrfunc}
    \State $\simulantennas[\enuser] \gets (\btantstr,\phyrecfields,\phyerrfunc)$
  \end{receive}
  \begin{receive}[\enidealfunc]{ShareExposure}{\enuser}
    \State $m \gets \simulincub/\simulchirpint$
    \State \SendAndReceive{Leak}{\enleakfunc}{\enidealfunc}{(\leaklcor,\leaklup)}
    \For{$(i*,j) \in leaklup$}
      \State find $(j,\protosec,\protomeas,\protochirp) \in \simulchirps$
      \State $\simulupseeds \gets \simulupseeds \concat \protosec$
    \EndFor
    \While{$|\simulupseeds| < m$}
      \State $\protosec \samuni \seedrange$
      \State $\simulupseeds \gets \simulupseeds \concat \protosec$
    \EndWhile
    \State \Return $\mathsf{Shuffle}{\simulupseeds}$
  \end{receive}
\end{simulator}

\paragraph{Simulator extension}
We extend the leak function to return the ciphertext for all data uploaded to TBB
\begin{simulator}{ext}
  \begin{receive}[\enidealfunc]{RegisterAuditor}{\enanalyst,\enanalfunc}
    \If{$\enanalyst \not\in\enanalysts$}
      \State \Send{Setup}{\enanalyst}{\fesr} (or simulate?)
      \State $\enanalysts[\enanalyst] \gets []$
    \EndIf

    \If{$\enanalfunc \in \enanalfuncset$}
      \State \Send{Keygen}{\enanalfunc,\enanalyst}{\fesr} (or simulate?)
      \State $\enanalysts[\enanalyst] \gets \enanalysts[\enanalyst] \concat \enanalfunc$
    \EndIf
  \end{receive}
  \begin{receive}[\enidealfunc]{Audit}{\enanalfunc,\enuser,y}
    %\If{$\party$ is corrupted}

    \If{$(\enuser,\enanalfunc) \in \enanalysts$}
    \State \SendAndReceive{Leak}{\enleakfunc}{\enanalfunc}{(\_,\_,\leaklsec)}
    \State \SendAndReceive{Decrypt}{\leaklsec}{\fesr}{\cdot} (or simulate)
    \State \SendAndReceive{Audit}{\enanalyst,\enanalfunc}{\enidealfunc}{y}
    \State \Return $y$
    \EndIf
  \end{receive}
  \begin{receive}[\enuser \in \enuserscorr  \text{ to } \fesr ]{Encrypt}{}
    \State FakeReality?
  \end{receive}

  \begin{receive}[\enuser \in \enuserscorr  \text{ to } \fesr ]{Decrypt}{f,ct}
   \State if function is an audit function and ct is the secret data (or a pointer to it)
   \State send audit
   \State otherwise execute normaly FESR dfecrypt
  \end{receive}
\end{simulator}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> main.tex <==
main-lncs.tex

==> preliminaries.tex <==
\section{Preliminaries}
\subsection{FESR}
\label{sec:fesr}
We recap the $\fesr$ ideal functionality,
first presented in \cite{PKC:BKMT21}. $\fesr$ is an extension over previous notions of
functional encryption, where the class of computable functions $\Ffamily$ can
capture statefulness and randomness: for each (decryptor,function) pair, the
functionality keeps a state which is updated over successive decryptions, and
fresh randomness is able to affect the computation.

The Functionality considers three types of entities: encryptors (known as $\PartyA$), decryptors (known as $\PartyB$) and Key generation authority ($\PartyC$). It provides procedures to Setup each type of party (besides $\PartyC$, which is generally assumed to be unique); to generate a functional key for a decryptor to compute a specific function; to encrypt a message $\fein$; and to compute a decryption of a message (given its handle and a valid functional key). We assume there exists a $\getHandle$ procedure that derives a unique identity.


\begin{functionality}{$\primname[\sid,\Ffamily,\PartyA,\PartyB,\PartyC$]}
	The functionality is parameterized by the randomized function class $\Ffamily$ such that for each $\funcF \in \Ffamily : \FfamilyDef$, over state space $\festates$ and randomness space $\ferand$,
  and by three distinct types of party entities $\PartyA,\PartyB, \PartyC$ interacting with the
  functionality via dummy parties (that
  identify a particular role). For
  each decryptor/function pair, a state value is recorded.
  \begin{statedecl}
  \statevar{\leakfunc}{}{Leakage function returning the length of the message}
%  \statevar{\Ffamily^+}{\Ffamily \setminus \{F_0\}}{}
	\statevar{\mathsf{setup[\cdot]}}{\false}{ Table recording which parties were initialized.}
  \statevar{\preimages[\cdot]}{\bot}{Table storing the plaintext for each message handler}
  \statevar{\partySet[\cdot]}{\bot}{Table of authorized functions and their states for all decryption parties}
  \end{statedecl}
  \begin{receive}[\text{party } \PartyC, \text{ for } \party \in \{\PartyA,\PartyB\}]{setup}{\party}  % TODO Should this take 1^{\lambda} parameter
     %\State $\texttt{setup} \gets \mathsf{true}$
     %\State $\forall \PartyB \in \PartyBS, R[\PartyB,F_0]\gets \vec{0}$
     \State $\mathsf{setup}[\party] \gets \mathsf{true}$
     \State \Send{setup}{\party}{\adversary}
  \end{receive}

  \begin{receive}[ \adversary, \text{ for } \party \in \{\PartyA,\PartyB\}]{setup}{\party}  % TODO Should this take 1^{\lambda} parameter
     \State $\mathsf{setup}[\party] \gets \mathsf{true}$
     \State $\partySet[\party,\leakfunc]\gets \initstate$
     \State \Send{setup}{}{\party}
  \end{receive}

	\begin{receive}[\text{party } \party \in \{\PartyA,\PartyB\}]{encrypt}{\fein}
      \If{$\mathsf{setup}[\party]=\mathsf{true} \land \fein \in \fedomain$}
      \State compute $\handle \gets \getHandle$
      \State $\preimages[\handle] \gets \fein$
      \State \Send{encrypted}{\handle}{\party}
    \EndIf
  \end{receive}
  \begin{receive}[\text{party } \PartyC]{keygen}{\funcF,\PartyB}
    \If{$\funcF \in \Ffamily^+ \land \mathsf{setup}[\PartyB]=\mathsf{true}$}
	  \State \SendAndReceive{keygen}{\funcF,\PartyB}{\adversary}{\msg{Ack}{}}
    \State $\partySet[\PartyB,\funcF] \gets \initstate$
	  \State \Send{assigned}{\funcF}{\PartyB}
    \EndIf
  \end{receive}
  \begin{receive}[\text{party } \PartyB]{decrypt}{\handle,\funcF}
    \State $\fein \gets \preimages[\handle]$
    %\If{$\PartyA$ and $\PartyC$ are honest}
    \If{$\PartyC$ is honest}
    \If{$ \partySet[\PartyB,\funcF] \neq \bot \land \fein \in \fedomain $}
	\State $\ferc \gets \ferand$
        \State $\festate \gets \partySet[\PartyB,\funcF]$
        \State $(\feout,\festate) \gets \funcF(\fein,\festate,\ferc)$
        \State $\partySet[\PartyB,\funcF] \gets \festate'$
        \State \Return $\msg{decrypted}{\feout}$
      \EndIf
    \Else
      \State \SendAndReceive{decrypt}{\handle,\funcF,\fein}{\adversary}{\msg{decrypted}{\feout}} % can the adversary change s,s' here?
      \State \Return $\msg{Decrypted}{\feout}$
    \EndIf
  \end{receive}
\end{functionality}

%assume M[h0] = empty


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> protocol.tex <==
\section{Protocol}
Our protocol assumes the following parties
\begin{itemize}
\item clients: smartphone or hardware tokens, bluetooth and GPS enabled; for simplicity, we assume a total of $N$ clients
\item server: central server, run by the national health authority or equivalent
\item certifier: local health authority or testing center, responsible for administering tests and certifying infection status on the system
\end{itemize}

Attacker model: the server is treated as honest-but-curious, wanting to learn the location history of any specific user; malicious clients might want to generate a fake map (possibly colluding), to change a specific area to be shown as (not) infected (lazy student attack).

\subsection{algorithm}
The heatmap generation is computed through the primitive of FESR.
To recap the semantics of Functional Encryption, this primitive allows a party who is in
possession of a function-specific key to compute a function on some encrypted
ciphertext, without learning its plaintext value. A message only needs to be
encrypted once, and several functions can be computed on it. In a practical
scheme such as Steel, we distinguish between three roles: the encryptor
(client), decryptor (server), and a Trusted Authority who generates public
parameters and the functional keys to distribute to decryptors.
For the purposes of our protocol, the Authority needs to be an entity that is trusted to set appropriate parameters for the decoding function outlined below. The authority can not collude with the server, otherwise privacy is trivially-violated (through authorisation of the identity function or similar).

\subsubsection{client}
The client runs the same application as DP-3T (or their local regional variation), but augmented with location tracking permission. The application will record the location of the client in the background, and store the amount of time spent in a specific area, using a well-defined encoding mechanism. Granularity of location collections (both spacial and temporal) are tradeoffs between accuracy and privacy/efficiency. Clients and Server operate using a mutually well-known encoding of the considered region into $k$ discrete bins. Whenever the user collects a location datapoint, they will increase by one the corresponding entry in the $k$-sized location history vector $x$. After the incubation window has elapsed (14 days for Covid-19), we can subtract those locations from $x$ again. The sum of all entries in $x$ should be equal to incubation window $\times$ collection frequency; whenever this is true, we say that $x$ is \textit{well-formed}.

Once the user of a client is tested and marked as infected by the certifier, through a digital signature $\sigma$ on their DP-3T seed $k$, they upload an encryption of $x,k,\sigma$ under the FESR master public key, along with their ephemeral ids for DP-3T.

\subsubsection{server}
The server, which processed normal DP-3T queries, also instantiates a Decryption enclave for Steel.
When initialising the system, the server contacts the trusted Authority to request authorisation to the following function:\\
- F-heatmap: \\
- on input($x,k,\sigma$): \\
- check that $x$ is well formed, and that $\sigma$ is a valid signature on $k$ from the health authorities \\
- append $x$ to matrix $Z$ \\
- if $Z$ size $>$ threshold t, return sum($Z$,col)\\

The server runs F-heatmap($x,k,\sigma$) on every encrypted trace uploaded by infected users. The return value for this function is a $k$-length vector holding the total count of ``infected time'' spent in each region by everyone who tested positive. This can be published as a heatmap for the last 14 days at the end of each day

(problem: we need the matrix to ``forget'' the input of 15 days ago, but keep the rest of that users' vector; solution: we actually send 14 different 24-hours vectors, produce 14 different matrices and then sum them?)
(problem: it's not clear how we bootstrap the health authorities signatures - same org as the FE trusted authority using a group signature?)
\subsection{geo-encoding}
\subsection{security}
Summing the rows of a matrix is a disruptive operation: given the final result, with enough data we can not reconstruct how individual users contributed to the final result. A small value of t, however, increases the probability of guessing. To prevent the server to bypass the threshold by feeding arbitrary inputs that would allow it to learn the honest users', it is necessary to check that the input was honestly signed by a health authority

\subsubsection{malicious client input}
Just as DP-3T, our protocol is susceptble to attacks from malicious clients. On a mobile device, GPS can be trivially spoofed, therefore we can't assume client inputs will be honestly generated
A simple measure that offers a little bit of mitigation for client-side attacks is to checksum the total weight of the matrix must equal to 24 (hours) * 14 (days) * $p$ (users), so an attacker that wants to alter the numbers in one region needs to also change those in another (if you increase the amounts of infected hours spent somewhere, you must decrease the ones spent somewhere else)
\subsection{...}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

